Towards Foundation Models for Mixed Integer Linear Programming

Mixed Integer Linear Programming (MILP) is essential for modeling complex decision-making problems but faces challenges in computational tractability and requires expert formulation. Current deep learning approaches for MILP focus on specific problem classes and do not generalize to unseen classes. To address this shortcoming, we take a foundation model training approach, where we train a single deep learning model on a diverse set of MILP problems to generalize across problem classes. As existing datasets for MILP lack diversity and volume, we introduce MILP-Evolve, a novel LLM-based evolutionary framework that is capable of generating a large set of diverse MILP classes with an unlimited amount of instances. We study our methodology on three key learning tasks that capture diverse aspects of MILP: (1) integrality gap prediction, (2) learning to branch, and (3) a new task of aligning MILP instances with natural language descriptions. Our empirical results show that models trained on the data generated by MILP-Evolve achieve significant improvements on unseen problems, including MIPLIB benchmarks. Our work highlights the potential of moving towards a foundation model approach for MILP that can generalize to a broad range of MILP applications. Our code and data are publicly available at https://github.com/microsoft/OptiGuide.

==> src/intro_submit.tex <==
\section{Introduction}
Mixed Integer Linear Programming (MILP) is a versatile mathematical framework widely used to model complex decision-making problems across various domains, including healthcare~\citep{eriskin2024robust}, supply chain management~\citep{kaya2016mixed}, energy systems~\citep{wouters2015energy}, and finance~\citep{mansini2015linear}. Its ability to represent intricate combinatorial structures and constraints makes it an indispensable tool in both academic research and industry applications.

Despite its widespread applicability, MILP faces two fundamental limitations. First, tractability is a major concern; solving MILP problems is computationally intensive and time-consuming, particularly for large-scale instances, due to the inherent NP-hardness. This complexity often results in long solve times, posing challenges for time-sensitive applications. Second, \slirebuttalblue{understanding the MILP formulation of an optimization problem} requires significant expertise in mathematical modeling and optimization, which limits accessibility for non-experts.
% formulating an optimization problem as a MILP

To address these challenges, researchers have attempted to leverage machine learning (ML) to enhance MILP solvers, such as learning heuristics to accelerate the solving process~\citep{gasse2019exact, khalil2016learning}. 
The underlying hypothesis for why ML may help in MILP is that in most real-world applications, the instances are coming from an unknown distributions, which, although hard to represent analytically, can be learned by deep neural networks.
Despite this plausibility, the state-of-the-art ML approaches have achieved limited generalizability due to difficulties in adapting learned models to unseen problems and handling distributional shifts. Most existing methods~\citep{prouvost2020ecole, gasse2022machine} focus on {\em specific} problem classes such as Set Cover, Capacitated Facility Location, or Maximum Independent Set, and train class specific models. Unfortunately, these problem specific models fail to perform well on different or more complex MILP instances~\citep{huang2024distributional}. For example, a model trained to help solve Set Cover instances may not generalize to  instances of slightly modified problem formulations (e.g., more constrained versions) as well as other problem classes, such as  Facility Location.  This lack of generalization hinders practical adoption in real-world applications where problem characteristics vary widely.
A concurrent work goes beyond the problem specific training approach~\citep{huang2024distributional}, but the authors consider training a joint model on a small number of selected classes (five), which limits its general applicability.

The state of ML adoption for MILP is in sharp contrast to areas like computer vision and NLP, where the fields have moved away from training problem or task specific models to general purpose foundation models trained on diverse and large-scale datasets that are capable of generalizing to a wide range of tasks.
There are several challenges towards building such general purpose foundation models for MILP, the chief among them being the lack of diverse and large-scale training data.
%First, there are no well-established benchmarks, similar to MATH or HumanEval (this line is double edged sword) that can capture the most important aspects of Mixed Integer Linear Programming problems. 
Reliance on limited datasets like MIPLIB~\citep{gleixner2021miplib} is insufficient to capture the vast diversity of MILP problems encountered in practice. 
More significantly, the distribution of the combinatorial structures of optimal solutions for MILP instances is more complex than the distribution of images or language, challenging the efficacy and development of general purpose foundation models.


Our work is motivated by the following questions:

{\em Do principles of foundation model training that have been so successful in NLP and vision modalities extend to the MILP modality?  Can a single model trained on diverse MILP problem classes generalize to unseen MILP classes?}

\input{src/teaser_fig}

\subsection{Our Contributions}
% This work answers these questions by showing an initial promise towards training foundation models for MILP. 
% Unlike previous works that trained a special purpose model for one or a few classes of MILP problems, we train a single model on diverse MILP problems, which can generalize to unseen classes.
% Towards that goal, our work builds on Large Language Models (LLMs)~\citep{achiam2023gpt, dubey2024llama, fewshotlearners} for generating larger and richer training data. The data are fed into Graph Neural Networks (GNNs), which have been shown to be effective in representing MILP instances \citep{gasse2019exact, scavuzzo2022learning, zhang2024towards}. This hybrid architecture enables us to capture the structural properties of MILP instances and learn representations that generalize across different problem classes. 

\slirebuttalblue{This work answers these questions by showing an initial promise towards training foundation models for MILP. We demonstrate that, a single model, trained on sufficiently diverse MILP problems, can effectively generalize to a variety of unseen MILP classes.} We develop a comprehensive framework that combines Large Language Models (LLMs)~\citep{achiam2023gpt, dubey2024llama, fewshotlearners} for generating larger and richer training data with Graph Neural Networks (GNNs), which have proven effective in representing MILP instances~\citep{gasse2019exact, scavuzzo2022learning, zhang2024towards}. This hybrid architecture can capture the structural properties of MILP instances and learn representations that generalize across diverse problem classes.


The main contributions of this work are highlighted as follows:



% On one hand, to fix the scarcity of data, we leverage frontier LLMs to enhance the diversity of MILP problem instances that enables creation of larger and richer training set. On the other, to solve our downstream tasks, we propose a new training paradigm  that treats MILP instances as a {\em new modality}. 



% that have demonstrated remarkable capabilities in understanding and generating human-like text, code, and mathematical reasoning~\citep{achiam2023gpt, roziere2023code, wei2022chain, yao2024tree}.

\begin{figure}[!t]
    \begin{center}
    \includegraphics[page=1, width=0.99\textwidth,  trim=15cm 0cm 0cm 0cm, clip]{figures/paper-figures.pdf}
    \end{center}
    \caption{An overview of our approach: Left—\pipeline{} pipeline. We design an evolutionary pipeline to leverage a Large Language Model to generate a diverse set of MILP classes. Right—the learning tasks. We design three learning tasks capturing different aspects of MILP to study the multi-class learning for MILPs. }
    \label{fig:pipeline}
% \vspace{-0.5cm}
\end{figure}


\textbf{MILP Tractability Tasks.} We study two tasks that capture  important aspects of MILP tractability in a multi-class learning setting.
First, we consider the problem of estimating the {\em integrality gap} (IG) of MILPs, defined as the difference between the optimal value of the MILP and its linear programming relaxation. Our second task, \textit{learning to branch}, is a sequential decision-making task aimed at accelerating MILP solvers by learning efficient branching strategies, a core technique for solving MILPs. While previous works have explored similar tasks~\citep{chen2023on, geng2023deep, gasse2019exact, zhang2024towards}, they primarily focused on training problem-specific models that could only generalize to small set of problem classes. In contrast, we train a single model that can solve each task across a broad range of MILP classes and problems.

%As a linear programming relaxation of an MILP can practically be solved in polynomial time, with an estimate of the IG one can efficiently extract an estimation of the optimal objective value. The IG also plays a key role in approximation algorithms and is a widely studied mathematical object for many resource allocation and decision problems. \\
% The IG of a MILP instance is defined as the difference between the value of integral optimum solution of the  MILP instance to the optimal value of linear programming relaxation. 
% We  note that a linear programming relaxation of an MILP instance can practically be solved optimally in polynomial time, hence with an estimate of the IG one can extract an estimation of the optimal objective value. 
% Besides its utility in predicting the optimal objective, the IG plays a fundamental role in the design of approximation algorithms and is a widely studied mathematical object for many resource allocation and decision problems. 

% In particular, we examine whether a learning scheme can imitate or even do better than  strong branching, a very powerful, yet computationally expensive branching technique~\citep{achterberg2007constraint}. 

%Both these tasks have been considered in the literature. 
% The IG prediction problem was considered by \cite{geng2023deep, chen2023on}, while 
% learning to branch has been studied in ~\cite{gasse2019exact, scavuzzo2022learning, zhang2024towards}.
% Figure \ref{fig:teaser:barplot} shows that our approach leads to significant improvement compared to SOTA.

% We show how GNNs can be used to imitate the strong branching expert to accelerate the MILP solving process, 

%\slired{Figure \ref{fig:tsne, fig:teaser:barplot} shows highlights of our results for these two tasks. 
%The results show that our techniques improve tractability by reducing solving times of MILP instances and providing quick estimates of the optimal solution value. }
\textbf{A Contrastive Learning Framework for Understanding MILP in Natural Language.} We further introduce a new learning task aimed at enhancing the interpretability of MILP instances.
\slirebuttalblue{This task tackles a significant challenge in MILP accessibility: many open-source MILP datasets and business scenarios provide only raw constraint and variable values, making them difficult to interpret without domain expertise. To address this challenge, we develop a contrastive learning approach that aligns MILP instance embeddings and natural language descriptions, which significantly outperforms direct interpretation attempts by LLMs like GPT-4o. This task complements the tractability tasks by lowering the entry barrier for non-experts and potentially aiding experts in designing specialized algorithms by deepening their understanding of optimization formulations.
%, achieving up to 77.62\% accuracy in 4-way classification tasks and 53.99\% in 10-way tasks. 
% This capability complements the MILP tractability tasks as the first step in the MILP solving pipeline: 
}

% Specifically, the task's goal is to align MILP instances with their corresponding natural language descriptions. To accomplish this, we adapt the CLIP framework~\citep{radford2021learning} to the MILP domain, treating MILP instances and language descriptions as distinct \emph{modalities} and aligning them via contrastive loss training.
% This capability is crucial for helping non-experts understand problem formulations and identify potential errors, complementing our other tasks fo- cused on MILP solving

% We tackle this problem by performing a contrastive loss training by treating MILP and natural language descriptions as different modalities similar to the CLIP framework \cite{radford2021learning}.

% Figure \ref{fig:teaser:barplot} shows experimental results on a benchmark dataset which we created for this task. We observe that
% using \pipeline{} gives substantial performance improvements.


\textbf{MILP-Evolve: A Scalable Framework for Generating Diverse MILP Data.}
As alluded earlier, unlike text and image modality, existing public MILP datasets lack diversity and volume. To address this limitation, we introduce \pipeline{}, a novel LLM-based data generation pipeline, which leverages frontier models to generate diverse MILP classes and instances from few example seed classes. \pipeline{} combines diverse prompting tailored to the MILP domain, along with parameter search and filtering, to generate a wide range of MILP classes resembling various real-world optimization scenarios. Figure \ref{fig:tsne} shows that MILP problems generated by our framework have rich diversity.
Quantitatively, our approach has enabled us to generate \emph{more than a thousand} different MILP problem classes, much more than any publicly available dataset.

% with around a million different instances in total

% As such, we believe that \pipeline{} can help advance future research in the intersection of ML and Optimization.  

% \item \textbf{Applying MILP-Evolve leads to substantial
% accuracy gains for all tasks.} Through extensive experiments, we show that \pipeline{} is an effective data augmentation method for multi-class MILP learning; models trained on the generated classes achieve significant improvements on both the held-out test set and MIPLIB. 
% Furthermore, by incorporating GNNs to treat MILP problems as a new modality for learning tasks, we enhance generalizability across diverse problem classes. 

\textbf{Substantial Multi-Class Learning Gains Across All Tasks.}  
Our extensive experiments demonstrate that \pipeline{} combined with our GNN-based learning framework are highly effective in improving multi-class MILP learning. Key results from the held-out test set include a 5.8x correlation improvement for Integrality Gap Prediction, a 1.92x accuracy improvement for MILP alignment, and a 1.42x improvement in the fraction of problems solved to optimum within the time limit for Learning to Branch (see Figure~\ref{fig:teaser:barplot}). 
% We briefly summarize our main results on the held-out testset: for Integrality Gap Prediction, we achieve a 58\% correlation, outperforming the SOTA that achieves only 10\% correlation. For the MILP alignment task, our method reaches an accuracy of 71\%, compared to 37\% from the SOTA. Furthermore, in the Learning to Branch task, we solve 71\% of problems within the fixed time limit, surpassing the SOTA that is at 50\% (see Figure~\ref{fig:teaser:barplot}). 
We further observe improved transfer learning to \slirebuttalblue{a separate \pipeline{} test set based on unseen problem classes, as well as on} the MIPLIB test set when pre-training on the enriched \pipeline{} dataset.
These results highlight the substantial performance gains of our models trained on diverse problem classes generated by \pipeline{}.  \slirebuttalblue{Our findings reveal key insights for advancing MILP learning: \textit{the diversity of training data has substantially greater impact on model performance than data quantity alone.} These insights, along with our study's broader contributions, represent significant progress towards foundation models for MILPs}.

% These results, combined with our framework's ability to benefit both optimization experts and non-experts, represent significant progress toward production-ready foundation models for MILP.  
% To facilitate future research in this direction, we are committed to open-sourcing our entire framework.

%\ishai{This is a bit too general. Can we provide one concrete result (say, our best one)?}

% Additionally, by incorporating GNNs to treat MILP problems as a new modality for learning tasks, we enhance generalizability across diverse problem classes.




\section{Formal Descriptions of MILP and Learning tasks}
% \subsection{}

% We formally define the class of MILP problems, and the learning tasks we study (and introduce) in this paper. 

\subsection{Mixed Interger Linear Programming (MILPs)}
MILP involves optimization problems where some decision variables are constrained to be integers, and relationships among variables are linear in the form of constraints and an objective function. A MILP problem is formulated as: 
\begin{equation}
x_{ILP}^* = \argmin\{c^\intercal x: Ax \leq b, x_j \in \mathbb{Z} \forall j \in I\},
\end{equation}
where $x \in \mathbb{R}^n$ is the vector of decision variables, $c \in \mathbb{R}^n$ is the cost vector, $A \in \mathbb{R}^{m \times n}$ and $b \in \mathbb{R}^m$ define the linear constraints, and $I \subseteq \{1, \dots, n\}$ indicates the indices of variables required to be integer-valued. MILP is extensively used to model complex decision-making problems involving both discrete choices and continuous variables, capturing applications in supply chain optimization, scheduling, network design, and resource allocation~\citep{duong2018mixed, floudas2005mixed, rieck2012mixed}. However, solving MILP problems is challenging due to their NP-hardness, leading to computational intractability for large-scale instances.



==> src/new_results_full_table.tex <==
% \begin{table}[!t]
% \caption{\slirebuttalblue{Learning to Branch. Transfer Learning Results on a Different Evolved Test Set Originating from Six Unseen Seed Classes. Initializing with the \ours{} pre-trained model yields the best performance on the unseen test set.}}
% \label{tab:new_results_full}
% \centering
% % \begin{minipage}[t]{0.48\textwidth}
% %     \subcaption[(a)]{Integrality Gap Prediction.}
% %     \centering
% %     \scalebox{0.87}{
% %     \begin{tabular}{ccc}
% %         \toprule
% %         & \textbf{Deviation ($\downarrow$)} & \textbf{Corr. ($\uparrow$)} \\
% %         \midrule
% %         \textbf{Mean}     & 33.07\%                  & 0.00     \\
% %         \textbf{Seed}     & 32.96\%                  & 0.10     \\
% %         \textbf{Seed + Param.} & 32.77\% & 0.07 \\
% %         \textbf{Seed + VAE} & 30.27\% & 0.26 \\
% %         \textbf{Ours - Attn.} & 20.82\%                  & 0.57   \\
% %         \textbf{Ours}     & \textbf{20.14\% }                   & \textbf{0.58 }    \\
% %         \bottomrule
% %     \end{tabular}
% %     }
% %     \label{tab:new_results_gap_prediction}
% % \end{minipage}
% % \hfill
% % \begin{minipage}[t]{0.51\textwidth}
% %     \subcaption[(c)]{Language-MILP Contrastive Learning.}
% %     \centering
% %     \scalebox{0.87}{
% %     \begin{tabular}{ccc}
% %         \toprule
% %          & \textbf{4-Way Acc. ($\uparrow$)} & \textbf{10-Way Acc. ($\uparrow$)} \\
% %         \midrule
% %         \textbf{Seed}           & 37.21\%          & 18.73\% \\         
% %         \textbf{Seed + Param.}  & 39.68\%          & 20.35\% \\         
% %         \textbf{Seed + VAE}     & 33.67\%          & 15.58\% \\         
% %         \textbf{Ours - Attn.}       & 70.41\%             & 52.76\% \\            
% %         \textbf{Ours}           & \textbf{70.54\%} & \textbf{54.17\%} \\
% %         \bottomrule
% %     \end{tabular}
% %     }
% %     \label{tab:new_results_contrastive_learning}
% % \end{minipage}\\
% % \vspace{0.2cm}
% \begin{minipage}[t]{\textwidth}     
%     \subcaption[(b)]{Prediction Accuracy: For each method, we report the accuracy and the top-5 accuracy with respect to the Strong Branching Experts.
%     } 
%     \centering
%     \scalebox{0.87}{
%     \begin{tabular}{ccc}
%         \toprule
%         & \textbf{Prediction Accuracy} & \textbf{Top 5 Accuracy} \\
%         \midrule
%         \textbf{Seed (GCN)}  &  23.11\% &  56.82\%              \\
%         \textbf{Seed + Param. (GCN)} & 27.87\%  & 68.32\% \\
%         \textbf{Seed + VAE (GCN)} & 25.25\% & 60.81\% \\
%         \textbf{Ours (GCN)}   & \textbf{30.71\%}  & \textbf{70.33\%}       \\
%         \bottomrule
%     \end{tabular}
%     }
%     \subcaption[(b)]{Solving Performance: For each method, we report the proportion of instances solved to optimal within a $200s$ time limit (including network overhead); among those instances, we report the 1-shifted geometric mean of time improvement over SCIP Default including and excluding (Ex.) the network overhead (See Appendix~\ref{sec_appendix:learning_branch}).} 
%     \scalebox{0.87}{
%     \begin{tabular}{cccc}
%         \toprule
%         & \textbf{Time Improv. ($\uparrow$)} & \textbf{Time Improv. (Ex) ($\uparrow$)} & \textbf{\% Instances Solved to Optimal ($\uparrow$)} \\
%         \midrule
%         \textbf{Seed (GCN)}  &  -30.65\% &  -16.60\% &    49.59\%              \\
%         \textbf{Seed + Param. (GCN)} & -3.70\%  & 5.89\% & 64.52\% \\
%         \textbf{Seed + VAE (GCN)} & -26.18\% & -13.50\% & 49.06\%\\
%         \textbf{Ours (GCN)}   & \textbf{15.49\%}  & \textbf{21.02\%}       &  \textbf{70.90\%} \\
%         \bottomrule
%     \end{tabular}
%     }
%     \label{tab:new_results_branching}
% \end{minipage}
% \end{table}
